Decade Long Timing Study of the Black Widow Millisecond Pulsar J1544+4937

Results from 11 years of radio timing for eclipsing black widow millisecond pulsar (MSP) binary, J1544+4937, is presented in this paper. We report a phase-connected timing model for this MSP, using observations with the Giant Metrewave Radio Telescope (GMRT) at multiple frequencies and with Green Bank Telescope (GBT). This is the longest-duration timing study of any galactic field MSP with the GMRT. While extending the timing baseline from the existing 1.5 years to about a decade we report the first detection for a significant value of proper motion ($\mathrm{\mu_{T}} \sim$ 10.14(5) $\mathrm{mas/year}$) for this pulsar. Temporal variations of dispersion measure ($\mathrm{\Delta DM~ \sim 10^{-3}}$ pc $\mathrm{cm^{-3}}$) manifested by significant determination of 1st, 2nd, and 3rd order DM derivatives are observed along the line of sight to the pulsar. We also noticed frequency-dependent DM variations of the order of $\mathrm{10^{-3}~ pc~ cm^{-3}}$, which could arise due to spatial electron density variations in the interstellar medium. This study has revealed a secular variation of the orbital period for this MSP for the first time. We investigated possible causes and propose that variation in the gravitational quadrupole moment of the companion could be responsible for the observed temporal changes in the orbital period.

==> J1544_timing_paperR1 (Version 2035)/table1.tex <==
\begin{table*}[!htb]
\begin{center}
\caption{Summary of the observations.}
\label{tab:Table1}
\vspace{0.3cm}
\label{discovery}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Backend       & $T_{res}^{a}$ & $F_{res}^{b}$ & Bandwidth & S$_{min}$ & Span &  ${\sigma_{\tiny  TOA}}$ \\
&($\mu$s)&(MHz)&(MHz) &(mJy)&& ($\mu$s)\\
\hline
Legacy GMRT$^{\ast}$  & 61 & 0.064 & 33 & $0.05^{c}$            & 2011$-$2017 &   $2.5^{d}$          \\
\hline
GBT$^{\dagger}$  & 81 & 0.024 & 100 & 0.09$^{i}$            & 2012 &         3$^{j}$    \\
\hline
Upgraded GMRT$^{\ast\ast}$ & 81 & 0.048 & 200 & $0.02^{c}$               &  2018$-$2022 & $1^{d}$        \\
\hline
\end{tabular}
\end{center}
$^{\dagger}$ : \cite{guppi}\\
$^{\ast}$ : \cite{roy2010real}\\
$^{\ast\ast}$ : \cite{gupta2017upgraded} \\
$^{a}$: Time resolution\\
$^{b}$: Frequency resolution\\
$^{c}$: 5$\sigma$ detection sensitivity calculated using the radiometer equation \citep{LorimerKramer} considering  gain of 0.32 K/Jy for the Legacy GMRT system and 0.38 K/Jy for the upgraded GMRT system, system temperature $\sim$ 123 K including the sky temperature in the direction of J1544+4937, 20\% duty cycle, 25 antennas ($\sim $ number of antennas used in the observations), considering 2 polarisation's and 60 mins of observing time in coherent array mode.\\
$^{d}$: Error in TOA estimation calculated using the radiometer equation considering the above parameters for GMRT in 10 mins of observing time at 400 MHz.\\
$^{i}$: 5$\sigma$ detection sensitivity calculated using the radiometer equation \citep{LorimerKramer} considering  gain of 2 K/Jy, system temperature is around 65 K at the position of the pulsar including all effects, considering 2 polarisations and 60 mins of observing time.\\
$^{j}$: Error in TOA estimation calculated using the radiometer equation considering the above parameters for GBT in 10 mins of observing time at 350 MHz.\\

\vspace{1cm}
\end{table*}

==> J1544_timing_paperR1 (Version 2035)/table2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{landscape}
\begin{table*}
%\begin{sidewaystable}
%\begin{table}
\centering
{\footnotesize
\caption{Timing parameters for PSR J1544+4937 using ELL1 and BTX model.
\label{tab:Table2}}
\begin{tabular}{|l|c||c|}
\hline
Model & ELL1 & BTX  \\
  \hline
 Timing Data Span     \dotfill           &55713.6$-$59622.2 & 55713.6$-$59622.2 \\
 Period epoch (MJD)\dotfill           & 55977.0 & 55977.0 \\
 Total time span (year) \dotfill                                & 10.7                         & 10.7              \\
 Number of TOAs\dotfill  &866 & 866 \\
 Reduced Chi-square \dotfill       &  7.5065       &  4.8642\\
 Post-fit residual rms ($\mu$s)\dotfill       & 6.942  & 5.578  \\
 \hline
 Right ascension (J2000)\dotfill &
 15$^\mathrm{h}$44$^\mathrm{m}$04\fs4911(1) &
 15$^\mathrm{h}$44$^\mathrm{m}$04\fs49135(9) \\
 Declination (J2000)\dotfill     &
 $+$49\degr37\arcmin55\farcs374(1) &
 $+$49\degr37\arcmin55\farcs3748(9)  \\
 Proper motion in RA (mas year$^{-1}$)\dotfill &$-$4.46(5) & $-$4.54(4) \\
 Proper motion in DEC (mas year$^{-1}$)\dotfill &$-$9.15(6) & $-$9.06(5) \\
 Spin frequency $f$ (Hz)\dotfill &
 463.11553585637(2) & 463.11553585640(1)\\
 Spin frequency derivative $\mathrm{\dot{f}}$ (Hz s$\mathrm{^{-1}}$)\dotfill &
 $-$5.998(1)$\times$10$^{-16}$  &
 $-$5.9996(9)$\times$10$^{-16}$ \\
Dispersion measure $\mbox{DM}$ (pc~cm$^{-3}$) &  23.2246(1)       & 23.22442(9) \\
 DM $1^{\mathrm st}$derivative $\mbox{DM1}$ (pc~cm$^{-3}$ year$^{-1}$) \dotfill & 0.00095(5)    & 0.00115(4)\\
DM $2^{\mathrm nd}$ derivative $\mbox{DM2}$ (pc~cm$^{-3}$ year$^{-2}$)\dotfill & $-$ 0.00041(2)   & $-$ 0.00048(1)\\
DM $3^{\mathrm nd}$ derivative $\mbox{DM3}$ (pc~cm$^{-3}$ year$^{-3}$)\dotfill & 5.9(4) $\times$ $10^{-5}$   & 7.08(3) $\times$ $10^{-5}$\\
 Orbital period $\mathrm{P_{b}}$ (days)\dotfill & 0.12077298998(8)  &  \\
 Orbital frequency FB0 \dotfill & & 9.58332993(2) $\times$ $10^{-5}$\\
 Orbital period 1st derivative (s/s)\dotfill & 6.6(4) $\times$ $10^{-13}$ & \\
 Orbital frequency $1^{\mathrm st}$derivative FB1 \dotfill & $-$ & 1.7(1)$\times$ $10^{-19}$  \\
 Orbital frequency $2^{\mathrm st}$derivative FB2 \dotfill & $-$ &-1.26(9)$\times$ $10^{-26}$ \\
 Orbital frequency $3^{\mathrm st}$derivative FB3 \dotfill & $-$ & 3.9(3)$\times 10^{-34}$\\
 Orbital frequency $4^{\mathrm st}$derivative FB4 \dotfill & $-$ & -6.3(5)$\times 10^{-42}$ \\
 Orbital frequency $5^{\mathrm st}$derivative FB5 \dotfill & $-$ & 4.4(3) $\times 10^{-50}$\\
 Projected semi-major axis $\mathrm{x}$ (lt-s) & 0.0328665(4) & 0.0328656(3) \\
 Time of ascending node $\mathrm{T_{ASC}}$ (MJD)\dotfill & 56124.7700998(4) & $-$\\
 $\mathrm{\epsilon_1 (e\cos{\omega})}$ \dotfill & 0.00003(2) & $-$  \\
 $\mathrm{\epsilon_2 (e\sin{\omega}})$ \dotfill & 0.00009(2) & $-$  \\
Eccentricity (e) \dotfill & 0.00010 & 5(1)$\times 10^{-5}$ \\ 
Epoch of periastron $\mathrm{T_{o}}$ (MJD) \dotfill & 56124.7765260 & 56124.7701015(4) \\
Longitude of periastron,  $\mathrm{\omega}$ (\degr) \dotfill & 19.15  & 0\\
 \hline
 \multicolumn{3}{c}{Derived parameters} \\
  \hline
 Galactic longitude, $\mathrm{l}$ (\degr) \dotfill    &  207.65 & 207.65 \\
 Galactic latitude, $\mathrm{b}$ (\degr) \dotfill    & 65.88 & 65.88  \\
 DM distance (kpc) \dotfill              & 1.2 $^\dagger$                        & 1.2$^\dagger$ \\
 & 2.9$^\ddagger$ & 2.9$^\ddagger$\\

 Observed $\mathrm{\dot{P}}$, $\mathrm{\dot{P}_{\rm obs}}$ ($\mathrm{s\, s^{-1}}$) \dotfill                             & 2.7966(5) $\times 10^{-21}$& $2.79735(4)\times 10^{-21}$  \\
 Intrinsic $\mathrm{\dot{P}}$, $\mathrm{\dot{P}_{\rm int}}$ ($\mathrm{s\,s^{-1}}$) \dotfill                             & 8.1 $\times 10^{-22}$ & $ 8.1 \times 10^{-22}$  \\
 Energy loss rate $\mathrm{\dot{E}}$ ($10^{33} \rm \, erg \, s^{-1}$)\dotfill                   &  12       &  12 \\
 Characteristic age, $\mathrm{\tau_c}$ (Gyear)\dotfill                &  42         & 42 \\
 Surface magnetic field, $\mathrm{B_0}$ (Gauss)\dotfill      &  $4.2 \times 10^{7}$         & $4.2 \times 10^{7}$ \\
 Total proper motion, $\mathrm{\mu_{T}}$ (mas year$^{-1}$) \dotfill       & 10.18(6)     & 10.14(5)  \\
 Companion mass, $\mathrm{M_c}$  (M$_{\odot}$)      \dotfill                           & 0.01697$<$ 0.0196 $<$ 0.0393 &  0.01697 $<$ 0.0196 $<$ 0.0393\\\hline
\end{tabular}
%\end{table}
}\\
{\small $^\ast$ Errors correspond to 1$\sigma$.\\
$^\dagger$ using the NE2001 model electron density distribution\\
$^\ddagger$ using the YMW16 model of electron distribution\\
%$^\ddagger$ using the \cite{} model of electron distribution\\
We note that the calculated DM distance is model dependent.\\
Timing uses DE405 solar system ephemeris.\\
The numbers in the parenthesis are uncertainties in preceding digits.}
%\end{sidewaystable}
\end{table*}
%\end{landscape}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


